Real-Fake: Effective Training Data Synthesis Through Distribution Matching

Synthetic training data has gained prominence in numerous learning tasks and scenarios, offering advantages such as dataset augmentation, generalization evaluation, and privacy preservation. Despite these benefits, the efficiency of synthetic data generated by current methodologies remains inferior when training advanced deep models exclusively, limiting its practical utility. To address this challenge, we analyze the principles underlying training data synthesis for supervised learning and elucidate a principled theoretical framework from the distribution-matching perspective that explicates the mechanisms governing synthesis efficacy. Through extensive experiments, we demonstrate the effectiveness of our synthetic data across diverse image classification tasks, both as a replacement for and augmentation to real datasets, while also benefits such as out-of-distribution generalization, privacy preservation, and scalability. Specifically, we achieve 70.9% top1 classification accuracy on ImageNet1K when training solely with synthetic data equivalent to 1 X the original real data size, which increases to 76.0% when scaling up to 10 X synthetic data.

==> table/Ablation2_Prompt.tex <==
\begin{table}[h]
\centering
\small
\caption{{\bf Ablation study} on prompting template components. We explore individual and combined effects on different prompt templates ( Base prompt, Image Caption, and Visual Guidance). The performance is evaluated with ImageNette and ImageNet100 top-1 classification accuracy.}
\label{tab:ablation2}
\begin{tabular}{ccc|cc}
\toprule
Base & Image Caption & Visual Guidance & ImageNette & ImageNet100  \\ 
\midrule
\Checkmark & & &  80.8 & 73.3 \\
\Checkmark & \Checkmark &  & 81.0 & 73.8 \\
\Checkmark & & \Checkmark  & 81.7 & 73.6 \\
\Checkmark & \Checkmark & \Checkmark & 82.3 & 74.0 \\
\bottomrule
\end{tabular}
\end{table}





==> table/AugmentDataset.tex <==
% % % EuroSAT
% \begin{table}[h]
%     \centering
%     \tablestyle{1.6pt}{1.0}
%     \caption{\textbf{Dataset Augmentation Performance}. + represents joint training with combined real and synthetic data. Top-1 and Top-5 image classification accuracy is reported.}
%     \begin{tabular}{l|llllllllllllll}
%     \toprule
%     & \multicolumn{1}{c}{IN-10} & \multicolumn{1}{c}{IN-100} & \multicolumn{1}{c}{IN-1K} & \multicolumn{1}{c}{CUB} & \multicolumn{1}{c}{Cars} & \multicolumn{1}{c}{PET} & \multicolumn{1}{c}{EuroSAT}\\
%     % & Top1 & Top5 & Top1 & Top5 & Top1 & Top5 & Top1 & Top5 & Top1 & Top5 & Top1 & Top5 & Top1 & Top5\\
%     \midrule
%     Real Data & 93.0 & 99.2& 86.3& 96.7& 79.6 & 94.6 & 81.5 & 95.6 &89.5 &98.5 &93.2 &99.5 &97.6 &99.9 \\
%     % + Baseline & 94.2 & 99.2&  87.0  & 97.2 & &  & &  & & &  & & & \\
%     + OURS & 95.1 \gain{2.1}& 99.4& 88.2 \gain{1.9}& 97.1 &79.9 \gain{0.3} & 94.8 & 83.5 \gain{2.0}& 96.1 & 90.3 \gain{0.8}& 98.7& 94.0 \gain{0.8} & 99.5 &98.9 \gain{1.3} &100.0 \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:your_label}
% \end{table}

% % EuroSAT
% \begin{table}[h]
%     \centering
%     \tablestyle{1.6pt}{1.0}
%     \caption{\textbf{Dataset Augmentation Performance}. + represents joint training with combined real and synthetic data. Top-1 and Top-5 image classification accuracy is reported.}
%     \begin{tabular}{l|llllllllllllll}
%     \toprule
%     & \multicolumn{1}{c}{IN-10} & \multicolumn{1}{c}{IN-100} & \multicolumn{1}{c}{IN-1K} & \multicolumn{1}{c}{CUB} & \multicolumn{1}{c}{Cars} & \multicolumn{1}{c}{PET} & \multicolumn{1}{c}{EuroSAT}\\
%     % & Top1 & Top5 & Top1 & Top5 & Top1 & Top5 & Top1 & Top5 & Top1 & Top5 & Top1 & Top5 & Top1 & Top5\\
%     \midrule
%     Real Data & 93.0 & 86.3& 79.6 & 81.5 &89.5 &93.2 &97.6 \\
%     % + Baseline & 94.2 & 99.2&  87.0  & 97.2 & &  & &  & & &  & & & \\
%     + OURS & 95.1 \gain{2.1}& 88.2 \gain{1.9}& 79.9 \gain{0.3} & 83.5 \gain{2.0} & 90.3 \gain{0.8} & 94.0 \gain{0.8} &98.9 \gain{1.3} \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:your_label}
% \end{table}

\begin{table}[t]
    \centering
    % \small
    \tablestyle{1.6pt}{1.0}
    \caption{\textbf{Dataset Augmentation Performance}. + represents joint training with combined real and synthetic data. Top-1 image classification \textit{\textbf{error rate}} is reported. The \textbf{\textit{relative improvements}} in percentage are rendered in \textcolor{Green}{green}.}
    \begin{tabular}{l|lllllll}
    \toprule
    & {ImageNet-10} & {ImageNet-100} & {ImageNet-1K} & {CUB} & {Cars} & {PET} & {EuroSAT} \\
    % & Top-1 Err & Top-5 Err & Top-1 Err & Top-5 Err & Top-1 Err & Top-5 Err & Top-1 Err & Top-5 Err & Top-1 Err & Top-5 Err & Top-1 Err & Top-5 Err & Top-1 Err & Top-5 Err\\
    \hline
    Real Data & $7.0$ & $13.7$ & $20.4$ & $18.5$ & $10.5$ & $6.8$ & $2.4$ \\
    % + Baseline$ & $94.2$ & $99.2& $ 87.0 $ & $97.2$ & $& $$ & $& $$ & $& $& $$ & $& $& $\\
    % \midrule
    % Baseline & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\
    % OURS & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\
    % \midrule
    + OURS & $4.9$\gainerr{30.0\%} & $11.8$\gainerr{13.9\%} & $20.1$\gainerr{1.5\%} & $16.5$\gainerr{10.8\%} & $9.7$\gainerr{7.6\%} & $6.0$\gainerr{11.8\%} & $1.1$\gainerr{54.2\%} \\
    \bottomrule
    \end{tabular}
    \label{tab:your_label}
\end{table}

==> table/CCPE_SyntheticOnly.tex <==
% \begin{wraptable}{l}{7cm}
%     \centering
%     % \footnotesize
%     \caption{\textbf{Synthetic Image Classification} Reported in form Top-1/Top-5 accuracy.}
%     \begin{tabular}{lcccc}
%     \toprule
%     & CUB & Cars & PET & EuroSAT \\
%     \midrule
%     Real Data & 81.5/95.6 & 89.5/98.5 & 93.2/99.5 & 97.6/99.9 \\
%     Baseline & 33.7/63.6 & 47.1/75.5 & 75.9/93.4 & 94.0/99.9 \\
%     OURS & 64.3/87.2 & 81.8/95.7 & 89.2/99.3 & 94.6/99.9 \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:ccpe_syn}
% \end{wraptable}

% \begin{table}[h]
%     \centering
%     \caption{\textbf{Synthetic Image Classification} Reported in form Top-1/Top-5 accuracy.}
%     \begin{tabular}{lcccc}
%     \toprule
%     & CUB & Cars & PET & EuroSAT \\
%     \midrule
%     Real Data & 81.5/95.6 & 89.5/98.5 & 93.2/99.5 & 97.6/99.9 \\
%     Baseline \ssy{missing reference} & 33.7/63.6 & 47.1/75.5 & 75.9/93.4 & 94.0/99.9 \\
%     OURS & 64.3/87.2 & 81.8/95.7 & 89.2/99.3 & 94.6/99.9 \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:ccpe_syn}
% \end{table}



% \begin{wraptable}{r}{0.6\textwidth}
%     \centering
%     \caption{\textbf{Synthetic Image Classification} Reported in form Top-1/Top-5 accuracy.}
%     \begin{tabular}{lcccc}
%     \toprule
%     & CUB & Cars & PET & EuroSAT \\
%     \midrule
%     Real Data & 81.5/95.6 & 89.5/98.5 & 93.2/99.5 & 97.6/99.9 \\
%     \makecell[l]{Baseline \\ \citep{Sariyildiz_2023_CVPR}}   & 33.7/63.6 & 47.1/75.5 & 75.9/93.4 & 94.0/99.9 \\
%     OURS & 64.3/87.2 & 81.8/95.7 & 89.2/99.3 & 94.6/99.9 \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:ccpe_syn}
% \end{wraptable}

% \vspace{-2mm}
\begin{wraptable}{r}{0.55\textwidth}
    \centering
    \tablestyle{3.6pt}{1.0}
    \caption{\textbf{Synthetic Image Classification Comparison.} Reported in Top-1 accuracy.}
    \begin{tabular}{lcccc}
    \toprule
    & CUB & Cars & PET & EuroSAT \\
    \midrule
    \ignore{Real Data} & \ignore{81.5} & \ignore{89.5} & \ignore{93.2} & \ignore{97.7} \\
    \hline
    \makecell[l]{Baseline\\ \citep{Sariyildiz_2023_CVPR}}   & 33.7 & 47.1 & 75.9 & 94.0 \\
    OURS & 64.3 & 81.8 & 89.2 & 94.6 \\
    \bottomrule
    \end{tabular}
    \label{tab:ccpe_syn}
\end{wraptable}

==> table/DeatailedSynApp.tex <==
\begin{table}[t]
    \centering
    \small
    \caption{
        \textbf{Image Classification Performance with Synthetic Data Only} Top-1 and Top-5 accuracies reported on three ImageNet datasets. Here \textit{w/} Real Images/Labels indicate the access to the real datasets \textit{when training the synthetic data generator}.
        % Img. and Lab. are abbreviations for Real Image and Label respectively, indicating the required information from real datasets. 
    }
    \begin{tabular}{l|c|cccccccccccc} % Added one more 'c' for the new column
        \toprule
          % & Model & \multicolumn{2}{c}{ImageNet-10} & \multicolumn{2}{c}{ImageNet-100} & \multicolumn{2}{c}{ImageNet-1K} & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{Cars} & \multicolumn{2}{c}{PET} & \multicolumn{2}{c}{EuroSAT} \\
          & \makecell[c]{\textit{w/} Real\\Images} & \makecell[c]{\textit{w/} Real\\Labels} & Model & \multicolumn{2}{c}{IN-10} & \multicolumn{2}{c}{IN-100} & \multicolumn{2}{c}{IN-1K} \\
          & & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5\\
        \hline
        \ignore{Real Data Training} &  & \ignore{93.0} & \ignore{99.2} & \ignore{86.3} & \ignore{96.7} & \ignore{79.6} & \ignore{94.6} & 81.5 & 95.6 &89.5 &98.5 &93.2 &99.5 &97.6 &99.9 \\
        BigGAN \citep{brock2018large} & BigGAN & -          & -     & -            & -     & 42.7      & 65.9   \\
        VQ-VAE-2 \citep{razavi2019generating} &  VQ-VAE & -          & -     & -            & -     & 54.8      & 77.6    \\
        CDM \citep{ho2022cascaded} & CDM & -          & -     & -            & -     & 63.0      & 84.1    \\
        FakeIt \citep{Sariyildiz_2023_CVPR} & SDv1.5  & -          & -     & 64.8         & 86.9  & 42.9       & 70.3     \\
        Imagen \citep{azizi2023synthetic} & Imagen & -          & -     & -            & -     & 69.2      & -        \\
        CiP \citep{lei2023image}  & SDv1.5  & 79.4       & -     & 62.4        & -     & 54.1      &   -       \\
        \hline
        % DiffDM (PI)   & P & SDXL V1.0  & 91.2      & 98.4  & 79.2         &  94.5     & 69.67      & 90.15    \\
        OURS  & SDv1.5 & 90.5       & 99.0  & 80.0         &  94.2     & 70.9      & 89.9    \\
        $\Delta$ \textit{with previous sota} & & \textcolor{Green}{+10.1} & - & \textcolor{Green}{+15.2} & \textcolor{Green}{+7.3} & \textcolor{Green}{+1.7} & - \\
        \bottomrule
    \end{tabular}
    \label{tab:app_detailed_synclassification}
    % \vspace{-4pt}
\end{table}

==> table/Face_gender.tex <==
\begin{table}[h]
\centering
\caption{CelebA Gender Classification Result Under Controlled Spurious Correlation. }
\label{tab:face_gender}
\begin{tabular}{l|ccc} 
\toprule
& I.I.D. & Flip & Random \\
\hline
Real Data & $93.40$ & $42.40$ & $68.80$ \\
\midrule
Baseline & $87.10$ & $72.60$ & $75.94$ \\
OURS & $90.44$ & $64.50$ & $71.69$ \\
\bottomrule
\end{tabular}
\end{table}
